Probing Higgs $CP$ properties at the CEPC

In the Circular Electron Positron Collider (CEPC), a measurement of the Higgs CP mixing through $e^{+} e^{-} \rightarrow Z H \rightarrow l^{+} l^{-}(e^{+} e^{-} /\mu^{+} \mu^{-}) H(\rightarrow b \bar{b} / c \bar{c} / g g)$ process is presented, with $5.6\ \mbox{ab}^{-1}$ $e^{+} e^{-}$ collision data at the center-of-mass energy of $240\ \mathrm{GeV}$. In this study, the CP-violating parameter $\tilde{c}_{Z \gamma}$ is constrained between the region of $ -0.30$ and $0.27$ and $\tilde{c}_{Z Z}$ between $-0.06$ and $0.06$ at $68\%$ confidence level. This study demonstrates the great potential of probing Higgs $CP$ properties at the CEPC.

==> tex/changelog.tex <==
\section{Changelogs}


\subsection{}
Updated 
\begin{itemize}
    \item Add new references in \ref{sec:1}.
    \item Update the definitions of angles in Appendix~\ref{appendix1}
    \item Change fast simulation to full simulation in \ref{sec:3}.
    \item Add ee event selection in \ref{sec:4}.
    \item Update all plots and tables.
    \item Add combined results and $20\ \mbox{ab}^{-1}$ results in \ref{sec:5_3}.
    \item Update the Abstract and Conclusion.
    
    {\color{blue}Tips: The blue part and all the graphs are the major update.}
\end{itemize}

